Simple Mechanisms for Welfare Maximization in Rich Advertising Auctions

Internet ad auctions have evolved from a few lines of text to richer informational layouts that include images, sitelinks, videos, etc. Ads in these new formats occupy varying amounts of space, and an advertiser can provide multiple formats, only one of which can be shown. The seller is now faced with a multi-parameter mechanism design problem. Computing an efficient allocation is computationally intractable, and therefore the standard Vickrey-Clarke-Groves (VCG) auction, while truthful and welfare-optimal, is impractical. In this paper, we tackle a fundamental problem in the design of modern ad auctions. We adopt a ``Myersonian'' approach and study allocation rules that are monotone both in the bid and set of rich ads. We show that such rules can be paired with a payment function to give a truthful auction. Our main technical challenge is designing a monotone rule that yields a good approximation to the optimal welfare. Monotonicity doesn't hold for standard algorithms, e.g. the incremental bang-per-buck order, that give good approximations to ``knapsack-like'' problems such as ours. In fact, we show that no deterministic monotone rule can approximate the optimal welfare within a factor better than $2$ (while there is a non-monotone FPTAS). Our main result is a new, simple, greedy and monotone allocation rule that guarantees a $3$ approximation. In ad auctions in practice, monotone allocation rules are often paired with the so-called Generalized Second Price (GSP) payment rule, which charges the minimum threshold price below which the allocation changes. We prove that, even though our monotone allocation rule paired with GSP is not truthful, its Price of Anarchy (PoA) is bounded. Under standard no overbidding assumption, we prove a pure PoA bound of $6$ and a Bayes-Nash PoA bound of $\frac{6}{(1 - \frac{1}{e})}$. Finally, we experimentally test our algorithms on real-world data.

==> lower_bounds.tex <==
\section{Lower bounds}\label{sec: lower bounds}
In this section we illustrate the challenge in coming up with allocation rules which are monotone in the set of rich ads. We also prove that monotonicity rules out approximation ratios strictly better than $2$ for deterministic mechanisms.

%provide some impossibility results that show that is not possible to obtain optimal allocation using a monotone allocation rule. 

\subsection{Simple algorithms fail}

% \anote{This is a good place to define bang-per-buck and incremental bang-per-buck}

%\amnote{A bit unclear what these different algorithms are: "optimal rule" (in Example 1), "incremental bpb algorithm" (in Example 2(i)), and "the 2-approx" (Example 2(ii)). }

 As we've already seen in Example~\ref{ex: opt}, the algorithm that finds the optimal integer allocation is not monotone. The following example shows that simple algorithms such as selecting ads in the incremental bang-per-buck order (as in Algorithm~\ref{alg:opt-greedy}), or the $2$ approximation algorithm presented in section ~\ref{subsec: fracopt} are not monotone either.
 %In fact simple algorithms such as selecting ads in the incremental bang-per-buck order (as in Algorithm~\ref{alg:opt-greedy}) can be non-monotone. %Which in particular means that the $2$ approximation algorithm presented in section ~\ref{subsec: fracopt} is not monotone. 
Recall that bang-per-buck = $b_{ij}/w_{ij}$ and incremental bang-per-buck = $\frac{b_{ij} - b_{ik}}{w_{ij} - w_{ik}}$ with $w_{ij} > w_{ik}$. Consider the following example:
\begin{example}
We have two advertisers $A$ and $B$. $A$ has two rich ads with (value, size) as (2,1),(3.5,3). $B$ has one ad with (value, size)=(3,3). %Suppose space $W \geq 3$, then the In this case, the two Pareto efficient integer allocations \amnote{I didn't understand what the Pareto allocs are -- there's no space fixed yet..} are 
%$\mathcal{A}_1 = {A: (2, 1), B: (3, 3)}$ and $\mathcal{A}_2 = {A: %(3.5, 3)}$. Advertiser A prefers the second allocation. 

% (i) Consider the algorithm that selects the allocation with the higher total value. In this example, it picks the allocation $\mathcal{A}_1$. However, if advertiser $A$ removes the rich ad $(2, 1)$, then the same algorithm picks the allocation $\mathcal{A}_2$. 

(i) Suppose the space is $W=4$. The incremental bang-per-buck algorithm is also not monotone. This algorithm allocates to the rich ad with the highest incremental bang-per-buck and stops when the next ad in the incremental bang-per-buck order is too big to fit in the remaining space. Thus, in the incremental bang-per-buck order, we will pick $A: (2, 1)$, followed by $B: (3, 3)$. The rich ad $A: (3.5, 3)$ does not get picked over $B: (3, 3)$, despite having higher bang-per-buck, since it has smaller incremental bang-per-buck (of $0.75$). On the other hand if A removes the rich ad $(2, 1)$, the algorithm picks $A: (3.5, 3)$ at the very beginning, and $A$ obtains a higher value.

(ii) Suppose $W = 3.5$, the optimal fraction solution (constructed by Algorithm~\ref{alg:opt-greedy}) is $A: (2, 1)$ with a weight of $1.0$ and $B: (3, 3)$ with weight $2.5/3$. The integer $2$-approximation algorithm from section~\ref{subsec: fracopt} will compare allocating just $A: (2, 1)$ or just $B: (3, 3)$ and select $B: (3, 3)$. But if A removed $(2, 1)$, then the optimal fraction solution is $A: (3.5, 3)$ with a weight of $1.0$ and $B: (3, 3)$ with weight $0.5/3$. The integer $2$-approximation algorithm will choose between $A: (3.5, 3)$ and $B: (3, 3)$ and select $A: (3.5, 3)$ because it has higher value. Thus A gets a higher value by removing $(2, 1)$. \footnote{In fact with this example even the fractional allocation is not monotone in fractional value. When A provides all rich ads its value is $2$, but when A removes $(2, 1)$, its value is $3.5$. Though to-be clear, we only seek integer monotone algorithms that always satisfy the knapsack constraint.}
\end{example}

% In general, it is hard to develop a monotone allocation algorithm that is even approximately optimal. For multiple other schemes motivated by the classic incremental-bang-per-buck $2$ approximation algorithm, it is possible to construct examples that break monotonicity.  \anote{add examples}
% On the other hand, algorithms that clearly satisfy monotonicity, e.g. selecting in the order of value, seem to achieve very poor approximation factors.

% randomizing because opt out to make your allocation better,
% lower bid to not end up the last one.
% % 
% \begin{itemize}
%     \item integral optimal allocation is not monotone.
%     \item incremental bang per buck is not monotone
% \end{itemize}

\subsection{An impossibility}
We first provide a lower bound on the approximation factor for any deterministic and monotone algorithms. 
\begin{theorem}
No deterministic and monotone algorithm has an approximation ratio better than $2 - \eps$, for any $\eps > 0$.
\end{theorem}
\begin{proof}
Consider an instance with two advertisers. Each advertiser has two rich ads: $(1, 1), (1+ \eps, 2)$. The total space available is $3$. In this example the optimal solution has value $(2 + \epsilon)$. 
To obtain an approximation better than $2-\epsilon$, 
the algorithm must choose a small ad for at least one of the advertisers. Since the algorithm is monotone in the set of rich ads, when that advertiser does not provide the small ad, the algorithm cannot switch to giving them the larger ad. Thus when the advertiser does not provide the small ad, the algorithm must give this advertiser nothing, which results in a social welfare of at most $(1+\eps)$. %Or when both bidders report their true value the algorithm should not allocate $(1, 1)$ to either which can result in a value of $(1+\eps)$ when the optimal is $2+\eps$. Thus any rich ad monotone allocation rule cannot obtain an approximation ratio better than $2$. 
\end{proof}

For randomized and monotone algorithms we show a bound of $12/11 - \eps$. {We include the proof of this lemma in Appendix~\ref{app: missing from lower bounds}.}

\begin{lemma}\label{lem: lower bound rand}
No randomized and monotone algorithm has an approximation ratio better than $12/11 - \eps$, for any $\eps > 0$.
\end{lemma}


